PASS-FC: Progressive and Adaptive Search Scheme for Fact Checking of Comprehensive Claims

Automated fact-checking (AFC) still falters on claims that are time-sensitive, entity-ambiguous, or buried beneath noisy search-engine results. We present PASS-FC, a Progressive and Adaptive Search Scheme for Fact Checking. Each atomic claim is first grounded with a precise time span and disambiguated entity descriptors. An adaptive search loop then issues structured queries, filters domains through credible-source selection, and expands queries cross-lingually; when necessary, a lightweight reflection routine restarts the loop. Experiments on six benchmark--covering general knowledge, scientific literature, real-world events, and ten languages--show that PASS-FC consistently outperforms prior systems, even those powered by larger backbone LLMs. On the multilingual X-FACT set, performance of different languages partially correlates with typological closeness to English, and forcing the model to reason in low-resource languages degrades accuracy. Ablations highlight the importance of temporal grounding and the adaptive search scheme, while detailed analysis shows that cross-lingual retrieval contributes genuinely new evidence. Code and full results will be released to facilitate further research.

==> section/app.tex <==
\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize, frame=single, breaklines=true]
[Definitions about Fact]
Fact: A fact is a statement or assertion that can be objectively verified as true or false based on empirical evidence or reality. 
Opinion: An opinion is a judgment based on facts, an attempt to draw a reasonable conclusion from factual evidence. While the underlying facts can be verified, the derived opinion remains subjective and is not universally verifiable. 
Atomic Factual Claim: An atomic factual claim is a statement that explicitly presents one verifiable fact. Statements with subjective components like opinions can also contain factual claims if they explicitly present objectively verifiable facts. 

[Instructions]
1. You are given a passage. Your task is to break the passage down into a list of atomic factual claims, based on the given [Definitions about Fact].
2. An atomic factual claim is a factual claim that cannot be decomposed. It only contains a singular piece of information.
3. Extract clear, unambiguous atomic factual claims to check from the input passage, avoiding vague references like 'he', 'she', 'it', or 'this', and using complete names. 
4. Please accurately identify and extract every claim stated in the provided text. Each claim should be concise (less than 15 words).

[Input Format Instruction]
<context>: Context for <passage> to help you understand it better.
<passage>: The passage to extract claims from.

[Output Format Instruction]
1. Your response MUST be a list of dictionaries. Each dictionary should contains the key "claim", which correspond to the extracted claim (with all coreferences resolved).
2. You MUST only respond in the format as described below. DO NOT RESPOND WITH ANYTHING ELSE. ADDING ANY OTHER EXTRA NOTES THAT VIOLATE THE RESPONSE FORMAT IS BANNED. START YOUR RESPONSE WITH '['.

[response format]: 
[
  {{
    "claim": "Ensure that the claim is fewer than 15 words and conveys a complete idea. Resolve any coreference (pronouns or other referring expressions) in the claim for clarity",
  }},
  ...
]

[Examples]
<context>: Who won the match between Tomas Berdych and Gael Monfis on Monte Carlo Masters, 2015?
<passage>: Tomas Berdych defeated Gael Monfis 6-1, 6-4 on Saturday. The sixth-seed reaches Monte Carlo Masters final for the first time. Berdych will face either Rafael Nadal or Novak Djokovic in the final.
<response>: [{{"claim": "Tomas Berdych defeated Gael Monfis 6-1, 6-4"}}, {{"claim": "Tomas Berdych defeated Gael Monfis 6-1, 6-4 on Saturday"}}, {{"claim": "Tomas Berdych reaches Monte Carlo Masters final"}}, {{"claim": "Tomas Berdych is the sixth-seed"}}, {{"claim": "Tomas Berdych reaches Monte Carlo Masters final for the first time"}}, {{"claim": "Berdych will face either Rafael Nadal or Novak Djokovic"}}, {{"claim": "Berdych will face either Rafael Nadal or Novak Djokovic in the final"}}]

<context>: How many photos does Tinder show by default, and can users access additional photos beyond this limit?
<passage>: Tinder only displays the last 34 photos - but users can easily see more. Firm also said it had improved its mutual friends feature.
<response>: [{{"claim": "Tinder only displays the last photos"}}, {{"claim": "Tinder only displays the last 34 photos"}}, {{"claim": "Tinder users can easily see more photos"}}, {{"claim": "Tinder said it had improved its feature"}}, {{"claim": "Tinder said it had improved its mutual friends feature"}}]

Now complete the following, ONLY RESPONSE IN A LIST FORMAT, NO OTHER WORDS!!!:
<context>: {prompt}
<passage>: {input}
<response>: 
\end{lstlisting}
\caption{The prompt used in Claim Decomposition.}
\label{prm:claim_decomp}
\end{figure*}


\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize, frame=single, breaklines=true]
[Definitions about Fact]
Fact: A fact is a statement or assertion that can be objectively verified as true or false based on empirical evidence or reality. 
Opinion: An opinion is a judgment based on facts, an attempt to draw a reasonable conclusion from factual evidence. While the underlying facts can be verified, the derived opinion remains subjective and is not universally verifiable. 
Atomic Factual Claim: An atomic factual claim is a statement that explicitly presents one verifiable fact. Statements with subjective components like opinions can also contain factual claims if they explicitly present objectively verifiable facts. 

[Instructions]
1. You are given a passage, a factual claim extracted from the passage, and a text feedback about the problem of the extracted claim. If the claim can be completely decomposed into multiple atomic factual claims, your task is to break the given factual claim down into a list of atomic factual claims, based on the given [Definitions about Fact]. Otherwise, return "None".
2. An atomic factual claim is a factual claim that cannot be decomposed. It only contains a singular piece of information.
3. If the feedback contains rational suggestions, they should be adopted to refine the final result.
4. Extract clear, unambiguous atomic factual claims to check from the given claim, avoiding vague references like 'he', 'she', 'it', or 'this', and using complete names. 
5. Please accurately identify and extract every claim stated in the provided text. Each claim should be concise (less than 15 words).

[Input Format Instruction]
<context>: Context for <passage> to help you understand it better.
<passage>: The passage where the following claim is extracted from.
<extracted_claim>: A claim that was extracted from the passage in a former round of claim extraction.
<feedback>: Feedback about the former round of claim extraction. It may contain problems about the extracted claim and corresponding suggestions.


[Output Format Instruction]
1. If the <extracted_claim> is already an atomic factual claim which cannot be further decomposed, output "None".
2. Otherwise, your response MUST be a list of dictionaries. Each dictionary should contains the key "claim", which correspond to the extracted claim (with all coreferences resolved).
3. You MUST only respond in the format as described below. DO NOT RESPOND WITH ANYTHING ELSE. ADDING ANY OTHER EXTRA NOTES THAT VIOLATE THE RESPONSE FORMAT IS BANNED. START YOUR RESPONSE WITH '['.

[response format]
[
  {{
    "claim": "Ensure that the claim is fewer than 15 words and conveys a complete idea. Resolve any coreference (pronouns or other referring expressions) in the claim for clarity",
  }},
  ...
]

[Examples]
{examples}

Now complete the following, ONLY RESPONSE IN A LIST OF DICTIONARIES FORMAT, NO OTHER WORDS!!!:
<context>: {prompt}
<passage>: {input}
<extracted_claim>: {claim}
<feedback>: {feedback}
<response>: 
\end{lstlisting}
\caption{The prompt used in Reflected Claim Decomposition.}
\label{prm:reflected_claim_decomp}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\tiny, frame=single, breaklines=true]
[Definitions]
1. Fact: A fact is a statement or assertion that can be objectively verified as true or false based on empirical evidence or reality. 
2. Atomic Factual Claim: An atomic factual claim is a statement that explicitly presents one verifiable fact. Statements with subjective components like opinions can also contain factual claims if they explicitly present objectively verifiable facts. 
3. Named Entity: A named entity is a real-world object, such as a person, location, organization, product, etc., that can be denoted with a proper name. It is a phrase that uniquely refers to an object by its proper name, acronym, or abbreviation.
4. Vague references are words or phrases that do not clearly specify their subject. These references may be clear in the original context but become ambiguous when the claim is isolated. Vague references include but are not limited to:
  - Pronouns (e.g., "his", "they", "her")
  - Unknown entities (e.g., "this event", "the research", "the invention")
  - Non-full names (e.g., "Jeff..." or "Bezos..." when referring to Jeff Bezos)

[Instructions]
1. You are given a <CLAIM> and its broader context, which includes a <PROMPT>, the <RESPONSE> to that prompt, and additional background information. The <CLAIM> is extracted from the <RESPONSE>, obeying the definiton of "Atomic Factual Claim" mentioned before.
2. Based on the given [Definitions], you need to first resolve vague references in the <CLAIM>, then augment the revised claim with its Time, and Named Entity information, ensuring each attribute helps to uniquely identify the fact and its context.
3. Requests for resolving vague references:
  a. Identify any vague references in the <CLAIM>.
  b. Replace these vague references with proper entities from the <RESPONSE> or context.
  c. Do not change any factual claims or add new information.
4. After resolving vague references, augment the revised <CLAIM> with the following background attributes based strictly on the information provided in the revised <CLAIM> and its context:
  a. Time: Specify the time when the fact in the claim holds true, based solely on the description in the revised <CLAIM> and its context. The "time" key represents the temporal context or validity period of the claim. It indicates when the statement is or was true, or from which point in time the information holds. This is crucial for facts that can change, such as political positions or current events. If there's no explicit time description in the claim or context, use "Now" as the default, indicating the fact is assumed to be true at present. Brief steps are:
    - If explicitly stated, use that time.
    - If not stated but implied, infer from context.
    - If no time information, use "Now".
  b. Entity: List named entities mentioned in the claim, providing brief but distinguishing descriptions based only on information given in the claim or context. It's because one named entity can refer to multiple objects. For instance, the city "Birmingham" could be "Birmingham, Alabama, USA" or "Birmingham, West Midlands, UK". Do not add any information that isn't explicitly stated or directly implied. Brief steps are:
    - List each entity in the claim.
    - Provide brief descriptions using only information from the claim or context.
5. Remember to maintain the original meaning of the claim while making it more precise and informative. The goal is to create a claim that is unambiguous and can be understood correctly even without additional context.
6. Before giving your revised statement, think step-by-step and show your reasoning. 

[Input Format Instruction]
<PROMPT>: Context for <RESPONSE> to help you understand it better.
<RESPONSE>: The passage where the following claim is extracted from. It's also the response of the former <PROMPT>.
<CLAIM>: The claim that was extracted from the <RESPONSE>. 

[Output Format Instruction]
You should only respond in format as described below. DO NOT RETURN ANYTHING ELSE. START YOUR RESPONSE WITH '{{'.
[response format]: 
{{
  "reasoning": "Find each vague reference. Explain what each vague reference likely refers to based on the claim and context. Show how you arrived at each conclusion. Then explain your reasoning for the Time attribute. Finally describe how you determined the Entity information.",
  "revised_claim": "Output the resolved claim.",
  "time": "The time when the fact in the claim holds true, using only information from the given claim and context.",
  ...
}}


[Examples]
<PROMPT>: You are a travel assistant. I will give you some reference documents of Singapore. Please output "Singapore's attraction introduction, mainly introducing the characteristics of attractions and what can be done here", output language must be English.
<RESPONSE>: Universal Studios Singapore, located within Resorts World Sentosa, is a cinematic adventure park that brings the silver screen to life with its thrilling rides and attractions . Each of its six themed zones offers a unique experience, from the prehistoric landscapes of The Lost World to the enchanting realm of Far Far Away . Visitors can immerse themselves in the futuristic Sci-Fi City, explore the mysteries of Ancient Egypt, or feel the buzz of New York and Hollywood's iconic streets . With 24 rides and attractions, including adrenaline-pumping roller coasters like Battlestar Galactica and family-friendly experiences such as the Madagascar river boat journey, there's something for every age and level of adventure . Live shows, character meet-and-greets, and a variety of dining and shopping options enhance the park's appeal, making it a must-visit destination for movie enthusiasts and thrill-seekers alike.
<CLAIM>: Universal Studios Singapore has six themed zones.
<OUTPUT>: {{"reasoning": "The subject in the claim is \"Universal Studios Singapore\", which is not a pronoun and does not reference an unknown entity. Furthermore, \"Universal Studios Singapore\" is not further specified in the RESPONSE, so we can assume that it is a full name. Therefore, there are not any vague references in the claim. The context did not include any specific time for its description. By default, we believe the RESPONSE still holds \"Now\". The entity \"Universal Studios Singapore\" need to be specified to avoid ambiguity.", "revised_claim": "Universal Studios Singapore has six themed zones.", "time": "Now", "Universal Studios Singapore": "located within Resorts World Sentosa, Singapore"}}


Now complete the following, ONLY RESPONSE IN A DICT FORMAT, NO OTHER WORDS!!!:
<PROMPT>: {prompt}
<RESPONSE>: {response}
<CLAIM>: {claim}
<OUTPUT>:
\end{lstlisting}
\caption{The prompt used in Claim Augmentation.}
\label{prm:claim_augment}
\end{figure*}


\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize, frame=single, breaklines=true]
[Definitions]
1. Google advanced search operators are special commands and characters that filter search results. 
2. Fact: A fact is a statement or assertion that can be objectively verified as true or false based on empirical evidence or reality. 

[Google Advanced Search Operators]
| Search operator | What it does                                      | Example                  |
|-----------------|--------------------------------------------------|--------------------------|
| " "             | Put any phrase in quotes to force Google to use exact-match. On single words, prevents synonyms. | "nikola tesla"      |
| OR              | Google search defaults to logical AND between terms. Specify "OR" for a logical OR (ALL-CAPS). | tesla OR edison           |
| -               | Put minus (-) in front of any term (including operators) to exclude that term from the results. | tesla -motors       |
| *               | An asterisk (*) acts as a wild-card and will match on any word. | tesla "rock * roll"       |
| ( )             | Use parentheses to group operators and control the order in which they execute. |(tesla OR edison) alternating current|
| before:         | Search for results from before a particular date. | apple before:2007-06-29  |
| after:          | Search for results from after a particular date.  | apple after:2007-06-29  |
| loc:            | Find results from a given area.                   | loc:"san francisco" apple |

[Instructions]
1. You and your partners are on a mission to fact-check a paragraph. Subclaims requiring verification have been extracted from the paragraph. Imagine yourself as an internet research expert. Your task is to generate two search queries for the provided claim to find relevant information for fact-checking.Please ensure that all queries are direct, clear, and explicitly relate to the specific context provided in the question and answer.
2. Utilize advanced Google search techniques when appropriate. But do not use site operators (e.g., site:example.com) in your queries, even if suggested in the feedback. Another tool will handle domain-specific searches separately.
3. Some searches have already been performed on this <CLAIM>. Please also consider the historical search information <HISTORY>. Adjust the queries based on the feedback from previous searches, focusing on areas where evidence was lacking or unclear.
4. Use date-based or location-based searches (before, after, and loc) only if: a) Historical search information is provided, AND b) The feedback in <HISTORY> explicitly indicates that the current search results are not within the required date range or destination.

[Output Format Instruction]
You should only respond in format as described below (a Python list of queries). PLEASE STRICTLY FOLLOW THE FORMAT. DO NOT RETURN ANYTHING ELSE. START YOUR RESPONSE WITH '['.
[response format]: ['query1', 'query2']

[Examples]
Here are three examples:
<CLAIM>: Michael Phelps is the most decorated Olympian of all time.
<RESPONSE>: ["Who is the most decorated Olympian of all time?", "Michael Phelps"]

<CLAIM>: Tesla is an American rock band formed in 1984.
<RESPONSE>: ["When is the rock band tesla formed?", "Rock band tesla Introduction. -motors -car -battery"]

<CLAIM>: Apple is used in various culinary applications. (The fruit apple)
<RESPONSE>: ["Apple's application in culinary. -phone -company", "Cooking ways of apple."]

Now complete the following(ONLY RESPONSE IN A LIST FORMAT, DO NOT RETURN OTHER WORDS!!! START YOUR RESPONSE WITH '[' AND END WITH ']'):
<CLAIM>: {input}
<HISTORY>: {feedback}
<RESPONSE>: 
\end{lstlisting}
\caption{The prompt used in Advanced Search.}
\label{prm:advanced}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize, frame=single, breaklines=true]
[Instructions]
1. You are an AI assistant tasked with verifying the truthfulness of a given claim. Your goal is to provide domain names of potentially relevant, credible, and authoritative sources while excluding unreliable sources. 
2. Only provide domain suffixes, not full URLs.
3. Include reliable sources such as:
  Government and official websites (.gov, .org)
  Encyclopedia websites (.wiki)
  Reputable news outlets (provide their official domain names)
4. Exclude unreliable sources like personal comments from forums or social media platforms.
5. If provided with a history of previous actions, which may include past searches and feedback. Focus on the search results and feedback.
  If official sources were found but didn't provide sufficient information, include them in your output for targeted searching
  If personal comments from forums were found, exclude those domains (mark with a minus sign, e.g., -reddit.com)
6. In summary, for each claim, provide:
  Recommended domain suffixes for searching
  Domains to exclude (marked with a minus sign)
  Any official sources from previous searches that warrant further investigation
7. You should only respond in format as described below (a Python list). PLEASE STRICTLY FOLLOW THE FORMAT. DO NOT RETURN ANYTHING ELSE. START YOUR RESPONSE WITH '['.
[response format]: ['url1', 'url2', '-url3']

[Examples]
<CLAIM>: The Eiffel Tower was built in 1889. 
<RESPONSE>: ['.gov.fr', '.paris.fr', '.unesco.org', .'britannica.com', '-tripadvisor.com', '-reddit.com']

<CLAIM>: COVID-19 vaccines are safe and effective. 
<RESPONSE>: ['.who.int', '.cdc.gov', '.nih.gov', '.edu', '-facebook.com', '-twitter.com']

<CLAIM>: Global temperatures have risen significantly in the past century.
<RESPONSE>: ['.nasa.gov', '.noaa.gov', '.ipcc.ch', '.nature.com', '-climatechangehoax.com', '-blogspot.com']

Now complete the following(ONLY RESPONSE IN A LIST FORMAT, DO NOT RETURN OTHER WORDS!!! START YOUR RESPONSE WITH '[' AND END WITH ']'):
<CLAIM>: {input}
<HISTORY>: {feedback}
<RESPONSE>: 
\end{lstlisting}
\caption{The prompt used in Site-Restricted Search.}
\label{prm:site}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize, frame=single, breaklines=true]
[Supported Languages]
["Afrikaans", "Amharic", "Bulgarian", "Catalan", "Chinese (Hong Kong)", 
"Chinese (PRC)", "Chinese (Taiwan)", "Croatian", "Czech", "Danish", 
"Dutch", "Estonian", "Filipino", "Finnish", "French (Canada)", 
"French (France)", "German", "Greek", "Hebrew", "Hindi", "Hungarian", "Icelandic", "Indonesian", "Italian", "Japanese", "Korean", "Latvian", 
"Lithuanian", "Malay", "Norwegian", "Polish", "Portuguese (Brazil)", 
"Portuguese (Portugal)", "Romanian", "Russian", "Serbian", "Slovak", 
"Slovenian", "Spanish (Latin America)", "Spanish (Spain)", "Swahili", 
"Swedish", "Thai", "Turkish", "Ukrainian", "Vietnamese", "Zulu"]

[Instructions]
1. You are an AI assistant tasked with analyzing claims and determining the most appropriate languages for fact-checking and evidence gathering. Your goal is to identify languages, other than English, that might provide more accurate, detailed, up-to-date, and factual evidence for a given claim.
2. When presented with a claim, analyze it for key elements such as locations, people, news sources, and event places. Based on these elements, determine if there are countries whose official languages might offer better sources of information. Consider that local languages often provide more detailed and accurate information.
3. If you identify relevant languages other than English, select up to two languages from the provided list that are most likely to yield valuable information. If only English is deemed suitable, do not output any languages, direct output None.
4. You should only respond in format as described below (a Python list of languages). Output None if only English is deemed suitable. PLEASE STRICTLY FOLLOW THE FORMAT. DO NOT RETURN ANYTHING ELSE. START YOUR RESPONSE WITH '['.
[response format]: ['language1', 'language2']

[Examples]
<CLAIM>: Angela Merkel announced her retirement from politics in 2021.
<RESPONSE>: ["German"]

<CLAIM>: Samsung unveiled its latest foldable smartphone at an event in Seoul. 
<RESPONSE>: ["Korean"]

<CLAIM>: The 2024 Carnival in Rio de Janeiro is expected to be the largest in history.
<RESPONSE>: ["Portuguese (Brazil)"]

<CLAIM>: Tensions between Russia and Ukraine escalated after the incident in the Kerch Strait.
<RESPONSE>: ["Russian", "Ukrainian"]

<CLAIM>: NASA's Perseverance rover discovered new evidence of ancient microbial life on Mars.
<RESPONSE>: None

Remember, the goal is to enhance fact-checking by identifying languages that might provide more comprehensive or accurate information than what's available in English sources alone.

Now complete the following:
<CLAIM>: {input}
<RESPONSE>:
\end{lstlisting}
\caption{The prompt used in Multilingual Search.}
\label{prm:multilingual}
\end{figure*}


\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize, frame=single, breaklines=true]
You are given a piece of factual claim. Your task is to identify whether there are any factual errors within the claim. Besides a claim, background information about the claim such as its valid time and descriptions of potentially confusing named entities is also provided. Note that the background information is only for better understanding of the claim. You SHOULD NOT judge the factuality of the background information.
        
Some evidence has already been retrieved in previous attempts to verify the claim, and several(at least one) verifications were made. The previous series of actions taken are saved in <STEP_HISTORY>. However, upon further reflection, it was discovered that there were issues with the previous verification process, and negative <FEEDBACK> was provided. The <FEEDBACK> includes an analysis of the problems with the previous attempt and a plan for the direction of future steps.
Based on the <FEEDBACK>, additional evidence may have been retrieved. If provided, please make good use of this <NEW_EVIDENCE>, along with the previous verification process stored in <STEP_HISTORY>, to verify the claim. If only the <FEEDBACK> is provided without new evidence, it means that the existing evidence in <STEP_HISTORY> is sufficient. You should follow the instruction in the <FEEDBACK> to identify and consider relevant evidence for re-verification.

When you are judging the factuality of the given text, you could reference the provided evidences if needed. The provided evidences may be helpful. You must be careful when using the evidence to judge the factuality of the given text. Supportive evidence should be consistent with the claim in terms of the facts, time, and named entities. Some evidence may contradict each other. But good evidence should comes from a credible source. If there is insufficient evidence to either support or refute the claim, classify it as INCONCLUSIVE.
The response should be a dictionary with four keys - "reasoning", "factuality", "error", and "correction", which correspond to the reasoning, whether the given text is factual or not (Boolean - True, False, or INCONCLUSIVE), the factual error present in the text, and the corrected text.

Now complete the following, ONLY RESPONSE IN A DICT FORMAT, NO OTHER WORDS!!!:
<CLAIM>:
{claim}
<STEP_HISTORY>:
{steps}
<FEEDBACK>:
{feedback}
<NEW_EVIDENCE>:
{evidence}
<OUTPUT>:
\end{lstlisting}
\caption{The prompt used in Claim Verification.}
\label{prm:verify}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize, frame=single, breaklines=true]
[Fact-checker's Action Process]
  1. Generate multiple questions to inquire about the truthfulness of key parts of the CLAIM.
  2. Search for information related to each question using a search engine.
  3. Based on the retrieved search results, determine if the CLAIM is truthful.  

[Tool Descriptions]
{descriptions}

[Instructions]
1. Please provide feedback on the series of actions taken by a fact-checker to verify a given CLAIM, and evaluate whether the final result is reasonable. If not, choose suitable tools for further improvement.
2. In your feedback, first comment on whether the evidence used adequately supports the conclusion and if the final result is reasonable. Provide positive feedback if everything looks good.
3. However, the conclusion may be 'INCONCLUSIVE' in determining the truthfulness of the CLAIM, or a wrong conclusion may have been reached. This is often due to insufficient evidence being collected, or existing evidence not being thoroughly analyzed, leading to overreliance on partial evidence (since the evidence is retrieved through search and is only related to the CLAIM being verified, it may not necessarily support or refute the CLAIM). In this case, provide negative feedback, suggest directions or plans for reformulating the questions, or provide new guidance for re-verification in the next step.
4. If negative feedback is given, specify tools to use next based on the tool descriptions. If no further verification is needed, output an empty list [] in the 'tool' field. There are two categories of tools:
  If additional evidence is needed, choose one or several question generation tools (aiming for a minimal sufficient set) to retrieve more relevant information. It's crucial to choose the specific sub-tools listed before, rather than the general 'generate_query' category, even if 'generate_query' appears in the action history. Any conbination of search tools is allowed. The search result of every selected tool will be considered as evidence. 
  If sufficient evidence exists but a new perspective is needed to notice relevant evidence for re-verification, select verification tools and put the new guidance for verification in the 'feedback' field. 

[Format Requirements] 
Please reply in the form of a dictionary with two keys, "feedback" and "decision". You should only respond in format as described below. DO NOT RETURN ANYTHING ELSE. START YOUR RESPONSE WITH '{{'.
{{
  "decision": "Boolean - True or False. Reply with True if re-verification is needed, or False if the process should end.",
  "tool": ["tool1", "tool2", "tool3", ...],
  "feedback": "It represents the textual feedback, analyzing the current issues. If there're any problems, give the direction for the next search to gather more adequate, relevant and reliable evidence. If only verification tool is selected, provide new guidance for re-verification in the next step here."
}}

Now complete the following, ONLY RESPONSE IN A DICT FORMAT, NO OTHER WORDS!!! START YOUR RESPONSE WITH '{{':
<CLAIM>:
{claim}
<STEP_HISTORY>:
{steps}
<OUTPUT>:
\end{lstlisting}
\caption{The prompt used in Feedback-Based Reflection.}
\label{prm:reflection}
\end{figure*}
